HexaGen3D: StableDiffusion is just one step away from Fast and Diverse Text-to-3D Generation

Despite the latest remarkable advances in generative modeling, efficient generation of high-quality 3D assets from textual prompts remains a difficult task. A key challenge lies in data scarcity: the most extensive 3D datasets encompass merely millions of assets, while their 2D counterparts contain billions of text-image pairs. To address this, we propose a novel approach which harnesses the power of large, pretrained 2D diffusion models. More specifically, our approach, HexaGen3D, fine-tunes a pretrained text-to-image model to jointly predict 6 orthographic projections and the corresponding latent triplane. We then decode these latents to generate a textured mesh. HexaGen3D does not require per-sample optimization, and can infer high-quality and diverse objects from textual prompts in 7 seconds, offering significantly better quality-to-latency trade-offs when comparing to existing approaches. Furthermore, HexaGen3D demonstrates strong generalization to new objects or compositions.

==> tables/inference_time_split.tex <==
\begin{table*}
    \centering
    \begin{adjustbox}{}
        {\renewcommand{\arraystretch}{1.2}
            \small
            \begin{tabular}{l|cccc}
            \hline
            \textbf{Method} & \multicolumn{4}{c}{\textbf{Latency (seconds)}} \\
            \multicolumn{1}{c|}{} & SDXL (20 steps) & SDXL (40 steps) & SD 1.5 (20 steps) & SD 1.5 (40 steps)
              
            \\ \hline
            
            text-to-hexaplane
                        & 1.65 $\pm$ \scriptsize{0.14} & 4.82 $\pm$ \scriptsize{0.14} & $\pm$ \scriptsize{} & $\pm$ \scriptsize{} \\
            hexaplane-to-triplane
                        & 0.08 $\pm$  \scriptsize{0.009} & 0.08 $\pm$ \scriptsize{0.009} & $\pm$  \scriptsize{} & $\pm$  \scriptsize{} \\
            triplane-to-mesh + vert. color
                        & 0.16 $\pm$  \scriptsize{0.001} & 0.16 $\pm$  \scriptsize{0.001} & $\pm$  \scriptsize{} & $\pm$  \scriptsize{} \\
            UV unwrapping
                        & 2.20 $\pm$  \scriptsize{0.77} & 2.15 $\pm$  \scriptsize{0.68} & $\pm$  \scriptsize{} & $\pm$  \scriptsize{} \\
            Texture baking
                        & 0.86 $\pm$  \scriptsize{0.05} & 0.86 $\pm$  \scriptsize{0.05} & $\pm$  \scriptsize{} & $\pm$  \scriptsize{} \\
            \hline
            \textbf{Total} 
                        & \cellcolor{tabfirst}4.97 $\pm$  \scriptsize{0.98} & \cellcolor{tabsecond}8.10 $\pm$  \scriptsize{0.89} & $\pm$  \scriptsize{} & $\pm$  \scriptsize{} \\

            \hline
            \end{tabular}
        }
    \end{adjustbox}
    \caption{We report the average latency with standard deviation of the main components in our proposed HexaGen3D model for text-to-3D generation with SDXL~\cite{podell2023sdxl} and StableDiffusion~\cite{rombach2022high} backbone text-to-image models for $20$ and $60$ denoising timesteps on NVIDIA A100 GPU with texture resolution of $1024 \times 1024$ on a set of $70$ text prompts.}
    \label{tab:latency_comparisons}
\end{table*}

==> tables/quantitative_comparison_openshape.tex <==
\begin{table}
    \centering
    \begin{adjustbox}{}
        \small
        {\renewcommand{\arraystretch}{1.1}
            \begin{tabular}{l|ccc}
            \hline
            \textbf{Method} & \multicolumn{3}{c}{\textbf{OpenShape}} \\
            \multicolumn{1}{c|}{} & Sim $\uparrow$ & Accuracy $\uparrow$ & Contrastive $\downarrow$
              
            \\ \hline
            
            MVDream-SD~\cite{shi2023mvdream}
                        & 7.77 & 28.3 & 4.05 \\
            TextMesh-SD~\cite{tsalicoglou2023textmesh}
                         & & & \\
            DreamFusion-SD~\cite{poole2022dreamfusion}
                            & 5.95 & 25.0 & 4.06 \\
            Shape-E~\cite{jun2023shap}
                        &  - & - & - \\
            \hline
            HexaGen3D-SD v1.5 %(40 steps)
                        & 10.25 & 70.0 & 4.02 \\ 
            HexaGen3D-SDXL %(40 steps)
                        & \cellcolor{tabfirst} 11.63 & \cellcolor{tabfirst} 76.7 & \cellcolor{tabfirst} 4.00 \\

            \hline
            \end{tabular}
        }
    \end{adjustbox}
    \caption{\mahesh{comparing methods on openshape metric}}
\end{table}

==> tables/quantitative_comparison_simple_prompts.tex <==
\begin{table*}
    \centering
    {\renewcommand{\arraystretch}{1.2}
        \small
        \begin{tabular}{l|ccc}
        \hline
        \textbf{Method} & \multicolumn{3}{c}{\textbf{R-Precision} $\uparrow$} \\
        \multicolumn{1}{c|}{} & CLIP B/32 & CLIP B/16 & CLIP L/14
          
        \\ \hline
        
        text-to-triplane SDv1.5
                    & 30.25 &  32.14 & 27.15 \\
        $^{\dagger}$unified SDv1.5
                    & \cellcolor{tabsecond}32.51 & \cellcolor{tabsecond}34.34 & \cellcolor{tabsecond}29.76 \\
        $^{\dagger}$unified SDv1.5 + hexaplane textures
                    & \cellcolor{tabfirst}33.18 & \cellcolor{tabfirst}34.63 & \cellcolor{tabfirst}30.13 \\
        $^{\ddagger}$unified SDXL
                    & 31.86 & 33.60 & 29.36 \\
        $^{\ddagger}$unified SDXL + hexaplane textures
                    & \cellcolor{tabthird}32.07 & \cellcolor{tabthird}33.85 & \cellcolor{tabthird}29.46 \\
        \hline
        \end{tabular}
    }
    \caption{Quantitative comparison on simple prompts.}
    \label{tab:quant_comparison_simple_prompts}
\end{table*}
